On Satisficing in Quantitative Games

Several problems in planning and reactive synthesis can be reduced to the analysis of two-player quantitative graph games. {\em Optimization} is one form of analysis. We argue that in many cases it may be better to replace the optimization problem with the {\em satisficing problem}, where instead of searching for optimal solutions, the goal is to search for solutions that adhere to a given threshold bound. This work defines and investigates the satisficing problem on a two-player graph game with the discounted-sum cost model. We show that while the satisficing problem can be solved using numerical methods just like the optimization problem, this approach does not render compelling benefits over optimization. When the discount factor is, however, an integer, we present another approach to satisficing, which is purely based on automata methods. We show that this approach is algorithmically more performant -- both theoretically and empirically -- and demonstrates the broader applicability of satisficing overoptimization.

==> Section/Probdef.tex <==




==> Section/intro.tex <==
\section{Introduction}
\label{Sec:intro}

%MYV2: Very rough.
Formal reasoning of systems are increasingly witnessing the combination of qualitative constraints with quantitative constraints. For instance, in planning and synthesis domains, these combinations are deployed to describe hard and soft constraints~\cite{lahijanian2015time}, obtain high-quality solutions~\cite{bloem2009better},  express constraints on cost and resource~\cite{he2017reactive}, 
%MYV2: Does not parse
even rewards in reinforcement learning~\cite{wen2016probably}, and the like.  
%MYV2: Does not parse
Existing literature has primarily focused on the problem of satisfaction of the qualitative goal while {\em optimization} of the quantitative goal. 
The issue, however, is that even the existence of solutions that meet both criteria cannot be determined~\cite{chatterjee2017quantitative,kwiatkowska2017prism}. As a result, current approaches trade-off between the two goals~\cite{chatterjee2017quantitative} and yet deliver weak theoretical guarantees w.r.t. both criteria (e.g.~\cite{wen2015correct}). 

%In addition to these limitations, solving the optimization problem can be expensive in practice, scaling to small-sized environment only. Thus limiting applicability of formal analysis techniques in planning/synthesis tasks~\cite{bloem2018graph}.


We argue that the optimal solution may not be required in several of these tasks.
For instance, a
solution with minimal battery consumption may be replaced by one that operates within the battery life; or a solution with optimal reward may be replaced by one that ensures a high-reward. 
Hence, many tasks can be reformulated to replace the optimization problem with an alternative form of quantitative analysis  wherein the problem is to search for a solution that adheres to a given threshold constraint. We call this the {\em satisficing problem}, a term popularized by H.A.Simon in economics to mean {\em satisfy and suffice} implying to obtain solutions that are good enough~\cite{satisficing}.


%To resolve these issues, we propose an alternate form of analysis in which the quantitative property is to search for a solution that adheres to {\em a given threshold constraint}.We refer to solving this quantitative property the {\em satisficing problem}, a well-established notion in economics that focuses on {\em good-enough} solutions~\cite{satisficing}. Our argument is that in several tasks optimal solutions may be replaced with satisficing ones. For instance, a solution with {\em minimal} battery consumption can be substituted by one that operates {\em within} the battery life. This work demonstrates the benefits of satisficing over optimization. 


The primary contribution of this work is to formulate and investigate the satisficing problem on 
two-player, finite-state games with the discounted-sum aggregate function as the cost model, which is a staple cost-model in decision making domains~\cite{osborne1994course,puterman1990markov,sutton1998introduction}. 
In these games, players take turns to pass a token along the {\em transition relation} between the states. As the token is pushed around, the play accumulates weights along the transitions using the  discounted-sum cost model. The players are assumed to have opposing objectives: one player maximizes the cost while the other player minimizes it. 
We define the satisficing problem as follows:  {\em Given a {\em threshold value $v \in \Q$}, does there exist a strategy for the minimizing (or maximizing) player that ensures the cost of all resulting plays is strictly or non-strictly lower (or greater) than the threshold $v$?} We exhibit several benefits of the satisficing problem in formal reasoning of systems, including strong guarantees on integration with temporal goals as well as algorithmic performance in theory and through empirical evaluations.


Towards the first benefit, we show that the satisficing problem can be efficiently reduced to solving a safety or reachability game when the discount factor is integral. Thus, integration of satisficing with temporal goals amounts to extension of the safety/reachability game obtained from reduction of satisficing with an $\omega$-regular objective obtained from the temporal goal (LTL~\cite{pnueli1977temporal,vardi1994reasoning}). Ultimately, solving satisficing with temporal goals via parity games~\cite{thomas2002automata}. This approach is guaranteed to produce solutions that fulfil both criteria, if they exist. 
Thus, in stark contrast to the lack of guarantees with optimization~\cite{chatterjee2017quantitative}. Furthermore, our approach applies beyond LTL to all kinds of $\omega$-regular specifications.


Our reduction of the satisficing problem applies {\em comparator automata} (comparator, in short) at its core~\cite{BCVFoSSaCS18}. So far, comparators have contributed theoretical and empirical progress in the discounted-sum inclusion problem~\cite{BCVFoSSaCS18,BCVCAV18,BVCAV19}. Our observation is that the criteria to fulfil  satisficing w.r.t. threshold value $v\in\Q$ can be expressed as membership in a comparator that accepts a weight sequence $A$ iff $\DSum{A}{d}$ $\mathsf{R}$ $v$ holds, where $d>1$ is the integer discount factor and $\mathsf{R} \in \{\leq, \geq, <,>\}$ is the relation. When the threshold value $v=0$, existing work shows that the comparator have compact representations as safety or co-safety automaton~\cite{kupferman1999model}. This paper extends these results to arbitrary but fixed threshold values $ v \in \Q$. By doing so, the criteria for satisficing can now be expressed as a safety or co-safety comparator automaton, and thus yield the reduction. 


Towards the second aspect of algorithmic performance, we demonstrate that satisficing has clear advantages over optimization with respect to theoretical complexity and empirical performance. For integer discount factors, our comparator-based approach  is solved in $\O(|V|+|E|)$, where $V$ and $E$ refer to the sets of states and transitions in the game. While the optimization problem is known to be solved in pseudo-polynomial time by a value-iteration (VI) based algorithm~\cite{hansen2013strategy,zwick1996complexity}, a thorough worst-case analysis of VI has  hitherto been absent. Therefore, we amend the oversight with a detailed analysis of VI for all discount factors $d>1$. First, we prove that VI can be terminated in $\Theta(|V|^2)$ iterations to compute the optimal value, as opposed to termination at infinitum. 
Next, since VI conducts several arithmetic operations in each iteration,  we account for their cost as well.
Its significance is  emphasised as we demonstrate orders of magnitude  of difference between the complexity of VI  under unit-cost and bit-cost models of arithmetic. For instance, when the discount factor is an integer, we show that VI  is $\O(|V|^2)\cdot |E|)$ and $\O(|V|^4\cdot |E|)$ under unit- and bit-cost model, respectively.
Clearly, satisficing fares better than VI. In fact, the fundamental separation between the two is  already apparent from the tight $\Omega(|V|^2)$ bound on the number of iterations.  

An empirically evaluation between our implementations of satisficing and VI supports the theoretical findings and shows that satisficing outperforms optimization. Additionally, it reveals that satisficing is displays robust performance, as opposed to VI, which is non-robust. 

\paragraph{Organization:}
We begin with preliminaries in \textsection~\ref{Sec:Prelims}.
\textsection~\ref{Sec:Satisfice} introduces and investigates the satisficing problem, our comparator-based solution, and its integration with temporal goals. \textsection~\ref{Sec:Optimization} presents the missing complexity analysis of VI for optimization. The algorithmic comparison of satisificing and VI is present in \textsection{}.

==> Section/satisficingzp.tex <==
\section{Satisficing via value iteration}
\label{Sec:VIForSatisfice}

So far, we have observed that for integer discount factors, comparator-based satisficing is more efficient than VI-based optimization. However, a crucial question still remains unanswered: Does the complexity improvement between VI for optimization to comparators for satisficing arise from (a) solving the decision problem of satisficing instead of optimization, or (b) adopting the comparator approach instead of numerical methods?
To answer this, we design and analyze a VI based algorithm for satisficing: If this algorithm shows improvement over VI for optimization, then the complexity gain would have occurred from solving satisficing. Otherwise, if this algorithm does not reflect any improvement, then the gain should  have come from adhering to comparator based methods. 

The VI based algorithm for satisficing is described as follows: Perform VI as was done for optimization in \textsection 3.1. Terminate the algorithm after whichever of the following two occurs first: (a) VI has performed the number of iterations as shown in Theorem~\ref{thrm:vsquareiterations}, or (b): In the $k$-th iteration, the threshold value $v$ falls outside of the interval defined in Lemma~\ref{lem:interval}.
In either case, one can determine how the threshold value relates to the optimal value, and hence determines satisficing. 


Clearly, termination by condition (a). results in the same number of iterations as optimization itself (Theorem~\ref{thrm:vsquareiterations}). We show that condition (b) does not reduce the number of iterations either.
On the contrary, it introduces {\em non-robustness} to the algorithm's performance (See \textsection~\ref{Sec:Intro}). The reason is that the number of iterations is based on the distance between the threshold value and the optimal value.
So, if this distance is large, few iterations will be required since the interval length in Lemma~\ref{lem:interval} declines exponentially. But if the distance is small (say close to 0), then it will take as many iterations as taken by optimization itself. Formally,
\begin{theorem}
\label{thrm:nonrobust}
Let $d >1$ be an integer discount factor. 
Let $G $ be a quantitative graph game with state set $V$. Let $\opt$ be the optimal cost, and  $v \in \Q$ be the threshold value. 
Then number of iterations taken by VI for satisfaction is $\min\{O(|V|^2), \log{\frac{\mu}{|W|-v}}\}$.
\end{theorem}
Hence, VI for satisficing does not improve upon VI for optimization. 
This indicates comparator-based methods may be responsible for the  improvement. 

